Optimal Best Arm Identification with Fixed Confidence in Restless Bandits

We study best arm identification in a restless multi-armed bandit setting with finitely many arms. The discrete-time data generated by each arm forms a homogeneous Markov chain taking values in a common, finite state space. The state transitions in each arm are captured by an ergodic transition probability matrix (TPM) that is a member of a single-parameter exponential family of TPMs. The real-valued parameters of the arm TPMs are unknown and belong to a given space. Given a function $f$ defined on the common state space of the arms, the goal is to identify the best arm -- the arm with the largest average value of $f$ evaluated under the arm's stationary distribution -- with the fewest number of samples, subject to an upper bound on the decision's error probability (i.e., the fixed-confidence regime). A lower bound on the growth rate of the expected stopping time is established in the asymptote of a vanishing error probability. Furthermore, a policy for best arm identification is proposed, and its expected stopping time is proved to have an asymptotic growth rate that matches the lower bound. It is demonstrated that tracking the long-term behavior of a certain Markov decision process and its state-action visitation proportions are the key ingredients in analyzing the converse and achievability bounds. It is shown that under every policy, the state-action visitation proportions satisfy a specific approximate flow conservation constraint and that these proportions match the optimal proportions dictated by the lower bound under any asymptotically optimal policy. The prior studies on best arm identification in restless bandits focus on independent observations from the arms, rested Markov arms, and restless Markov arms with known arm TPMs. In contrast, this work is the first to study best arm identification in restless bandits with unknown arm TPMs.

==> acknowledgements.tex <==
\section*{Acknowledgements}

The authors are supported by a Singapore National Research Foundation Fellowship (under grant number R-263-000-D02-281) and  by the  National Research Foundation, Singapore under its AI Singapore Programme (AISG Award No: AISG2-RP-2020-018).

==> iffalse-fi-parts.tex <==
In this section, we first present the test statistic and a threshold, based on which we subsequently present our stopping criterion. Recall from  \eqref{eq:parameter-estimates} that $\hat{\eta}(n) = (\hat{\eta}_a(n): a \in [K])$ denotes the estimates of the arm means at time~$n$. Let $\hat{\theta}_a(n) = \dot{A}^{-1}(\hat{\eta}_a(n))$ for each $a \in [K]$, and let ${\boldsymbol{\hat\theta}}(n) = (\hat{\theta}_a(n): a \in [K])$. Our test statistic at time $n$, denoted as $Z(n)$, is then defined as
\begin{equation}
    Z(n) \coloneqq \inf_{\boldsymbol{\lambda} \in \textsc{Alt}(\boldsymbol{\hat{\theta}}(n))} \sum_{(\underline{d}, \underline{i}) \in \mathbb{S}_R} \ \sum_{a = 1}^{K} N(n, \underline{d}, \underline{i}, a) \, D_{\text{KL}}(P_{\hat{\theta}_a(n)}^{d_a}(\cdot | i_a) \| P_{\lambda_a}^{d_a}(\cdot | i_a)).
    \label{eq:Z-of-n}
\end{equation}
Before we present the threshold, we introduce some notations. Let $K^\prime \coloneqq \sup_{\theta \in \Theta} \, \max_{i, j \in \mathcal{S}} \frac{v_\theta(j)}{v_\theta(i)}$, where $v_\theta$ is the left Perron--Frobenius eigenvector of the matrix $\tilde{P}_\theta$. From \cite[Proposition 1]{moulosanantharam2019optimal}, we have $K^\prime < +\infty$.\footnote{If $P(j|i)>0$ for all $i,j \in \mathcal{S}$, then we may set $K'=\max_{i,j,k}\frac{P(j|i)}{P(k|i)}$. If $P$ induces an i.i.d. process (i.e., $P$ has identical rows), then we may set $K'=1$. See \cite{moulos2019optimal,moulos2020concentration}.}  Furthermore, let $\gamma = \inf_{\theta \in \Theta} \min_{i \in \mathcal{S}} \mu_\theta(i)$. Recall $\Theta=[\theta_*, \theta^*]$. Because $\theta \mapsto \mu_\theta$ is continuous (Lemma~\ref{lem:important-properties-of-family}), and $\Theta$ is closed, it follows that the infimum in the expression for $\gamma$ is attained for some $\theta' \in \Theta$, and hence $\gamma = \min_{i \in \mathcal{S}} \mu_{\theta'}(i)>0$. 

\iffalse
Given $\delta \in (0,1)$, let 
\begin{equation}
    n_0 \coloneqq \inf\bigg\lbrace n \geq K: n^2 e^{-n} \leq \frac{\delta}{4KK^\prime \, e}\bigg\rbrace.
    \label{eq:n-0-definition}
\end{equation}
\fi

For any $\alpha>1$ and $\delta \in (0,1)$, our threshold at time $n$, denoted $\zeta(n, \delta, \alpha)$, is given by
\begin{equation}
    \zeta(n, \delta, \alpha) \coloneqq K \left(1+\frac{1}{\gamma}\right) \log \left(\frac{D\, n^\alpha}{\delta}\right),
    \label{eq:threshold-zeta}
\end{equation}
where $D=\frac{2\alpha\, K (K')^2}{\alpha-1}$.
%-------------------------------------------------------
\iffalse
\begin{equation}
    \zeta(n, \delta) \coloneqq \frac{K}{C_{\hat{\boldsymbol{\theta}}(n)}} \left[\frac{2\, n_0}{n_0-1} \log\log n + n_0\right],
    \label{eq:threshold-zeta}
\end{equation}
where
\begin{equation}
    C_{\hat{\boldsymbol{\theta}}(n)} \coloneqq \min_a \min_i \mu_{\hat{\theta}_a(n)}(i)>0.
    \label{eq:C-hat-theta-of-n}
\end{equation}
\fi 
Our stopping criterion is defined by the random variable
\begin{equation}
    \tau_{\delta} \coloneqq \inf\bigg\lbrace n \geq K: Z(n) \geq \zeta(n, \delta, \alpha) \bigg\rbrace.
    \label{eq:stopping-time}
\end{equation}
At stoppage, our recommendation $\hat{a}$ is the arm with the largest mean estimate, i.e., $\hat{a} = \argmax_a \hat{\eta}_a(\tau_{\delta})$.

















The following lemma demonstrates that under the proposed arms selection rule, the empirical fractions of $(\underline{d}, \underline{i}, a)$ tuples converge to the correct set of allocations.
\begin{lemma}
\label{lem:convergence-to-the-correct-set-of-optimal-allocations}
Under the proposed arms selection rule with $\eta \in (0,1)$, when $\boldsymbol{\theta} \in \Theta^K$ is the underlying instance, 
\begin{equation}
    \lim_{n \to \infty} d_{\infty}\left(\left\lbrace \frac{N(n, \underline{d}, \underline{i}, a)}{n} \right\rbrace_{(\underline{d}, \underline{i}, a)}, C_\eta(\boldsymbol{\theta}) \right) = 0 \quad \text{a.s.},
    \label{eq:convergence-to-the-correct-set}
\end{equation}
where $C_\eta(\boldsymbol{\theta}) \coloneqq \{\eta \, \nu^{\text{unif}}_{\boldsymbol{\theta}} + (1-\eta)\, \nu: \nu \in \mathcal{W}^\star(\boldsymbol{\theta}) \} $.
\end{lemma}

\iffalse
in a manner so that given any compact, convex set $C \subseteq \Sigma_R(\boldsymbol{\theta})$, we have
$$
\lim_{n \to \infty} d_{\infty} \left(\frac{N^{\text{active}}(n, \underline{d}, \underline{i}, a)}{n^{\text{active}}(n)}, \ C\right) = 0 \quad \text{a.s.}. 
$$
where $C_\eta = \{\eta \, \nu_{\boldsymbol{\theta}, R}^{\text{unif}} + (1-\eta)\, \nu: \nu \in C\}$.
From \eqref{eq:sampling-rule}, we note that arm $A_n=b_{n^{\text{active}}(n)}$ is selected only when $n^{\text{active}}(n) \geq K+1$. Thus, it suffices to specify $b_{n^{\text{active}}(n)}$ for $n^{\text{active}}(n) \geq K+1$.
\fi


\iffalse
The following result demonstrates that $\tau_{\delta}<\infty$ a.s. under the proposed arms selection rule.
\begin{proposition}
\label{prop:almost-sure-upper-bound}
For any $\boldsymbol{\theta} \in \Theta^K$, under the arms selection rule in \eqref{eq:sampling-rule} with parameter $\gamma \in (0,1)$, the stopping time $\tau_{\delta}$ is finite almost surely. Furthermore,
    \begin{equation}
        \limsup_{\delta \downarrow 0} \frac{\tau_{\delta}}{\log(1/\delta)} \leq  \frac{1}{\gamma \, T_R^{\text{unif}}(\boldsymbol{\theta}) + (1-\gamma)\, T_R^\star(\boldsymbol{\theta})} \quad \text{a.s.}.
        \label{eq:almost-sure-upper-bound}
    \end{equation}
\end{proposition}
\fi

\iffalse
Let $\pi_{R}^{\text{unif}}$ denote the policy that, for all $t\geq K$, selects the arms uniformly whenever the delay of each arm is $<R$, and forcibly selects an arm whose delay is equal to $R$. From \cite[Lemma 1]{karthik2022best}, we know that under $\pi_{R}^{\text{unif}}$, the process $\{(\underline{d}(t), \underline{i}(t)): t \geq K\}$ is an ergodic Markov process. Let $\mu_{\boldsymbol{\theta}, R}$ be the stationary distribution of the process $\{(\underline{d}(t), \underline{i}(t)): t \geq K\}$ under $\pi_{R}^{\text{unif}}$ and under the instance $\boldsymbol{\theta}$. 

\begin{lemma} [Arm Selection rule]
\label{lemma:forced-exploration}
Let $\{b_n: n \geq 1\}$ be any sequence of arms. For all $n \geq 0$, let $f(n) = \sqrt{n/K}$. Let $a_0=1, a_1=2, \ldots, a_{K-1} = K$, and let $\{a_n: n\geq K\}$ be defined recursively via 
\begin{equation}
    a_{n} = (a_{n-1}\ {\rm mod}\ K)+\mathbf{1}_{\left\lbrace\min_{a \in [K]} N(n, \underline{d}(n), \underline{i}(n), a) < f(n)\right\rbrace}, \quad n \geq K.
    \label{eq:i-n-recursive}
\end{equation}
Consider the arms selection rule given by $A_n=a_n$ for all $n \leq K-1$, and
\begin{equation}
    A_{n} = 
    \begin{cases}
        a, & (\underline{d}(n), \underline{i}(n)) \in \mathbb{S}_{R,a},\\
        a_{n}, & \min_{a \in [K]} N(n, \underline{d}(n), \underline{i}(n), a) < f(n) \text{ and } (\underline{d}(n), \underline{i}(n)) \notin \bigcup_{a=1}^{K} \mathbb{S}_{R,a},\\
        b_n, & \min_{a \in [K]} N(n, \underline{d}(n), \underline{i}(n), a) \geq f(n) \text{ and } (\underline{d}(n), \underline{i}(n)) \notin \bigcup_{a=1}^{K} \mathbb{S}_{R,a},
    \end{cases}
    \label{eq:sampling-rule}
\end{equation}
for all $n \geq 0$.
Then, under the arms selection rule in \eqref{eq:sampling-rule},
\begin{equation}
    \min_{a \in [K]} \ \min_{(\underline{d}, \underline{i}) \in \mathbb{V}_{R,a}} N(n, \underline{d}, \underline{i}, a) \geq f(n-K-1) \quad \forall \, n \text{ large}, \ a.s..
    \label{eq:forced-sampling}
\end{equation}
\end{lemma}
\fi

\iffalse
We now propose an arms selection rule that combines forced exploration via the $D$-tracking rule of \cite{garivier2016optimal} and uniform exploration of arms. To describe our algorithm, we introduce some notations. Given a fixed and positive constant $\eta \in (0,1)$, let $\{B_0, B_1, \ldots\}$ be a sequence of independent and identically distributed random variables following Bernoulli distribution with parameter $\eta$, independent of the arm selections and observations from the arms. For any $n \geq K$, let
\begin{equation}
    n^{\text{active}}(n) \coloneqq \sum_{t=K}^{n} \mathbf{1}_{\{B_{t-K}=0\}}
    \label{eq:n-active-of-n}
\end{equation}
denote the number of {\em active} instants up to time $n$. Further, let
\begin{equation}
    N_a^{\text{active}}(n) \coloneqq \sum_{t=K}^{n} \mathbf{1}_{\{B_{t-K}=0, \, A_t=a\}}
    \label{eq:N-a-active-of-n}
\end{equation}
denote the number of times arm $a$ is selected {\em actively} up to time $n$. We initialise $n^{\text{active}}(K-1)=0$ and $N_a^{\text{active}}(K-1)=0$ for all $a \in [K]$.

Let $\{b_1, b_2, \ldots\}$ be an arbitrary sequence of arms. For all $n \geq 0$, let $f(n) = (\sqrt{n} - K/2)_{+}$. 
\iffalse
Let $a_0 \coloneqq 0$, and let $\{a_1, a_2, \ldots\}$ be the sequence of arm selections defined via
\begin{equation}
    a_{n^{\text{active}}(n)} = (a_{n^{\text{active}}(n)-1}\ {\rm mod}\ K)+\mathbf{1}_{\left\lbrace\min_{a} N_a^{\text{active}}(n-1) < f(n^{\text{active}}(n))\right\rbrace}, \quad n^{\text{active}}(n) \geq 1, ~n \geq K.
    \label{eq:a-n-recursive}
\end{equation}

Let $a_1=1$, and let $\{a_n: n\geq 2\}$ be defined recursively via 
\begin{equation}
    a_{n+1} = (a_{n}\ {\rm mod}\ K)+\mathbf{1}_{\left\lbrace\min_{a \in [K]} N(n, \underline{d}(n), \underline{i}(n), a) < f(n)\right\rbrace}, \quad n \geq K.
    \label{eq:i-n-recursive}
\end{equation}
\fi
Our arms selection rule first selects $A_0=1, A_1=2, \ldots, A_{K-1}=K$. Thereafter, for all $n \geq K$, the arms selection rule works as follows.
\begin{enumerate}
    \item If $\max_a d_a(n)=R$, then select $A_n=\argmax_a d_a(n)$. Go to step 3. 
    \item If $\max_a d_a(n)<R$:
    \begin{itemize}
        \item If $B_{n-K}=1$, select $A_n$ uniformly at random. Go to step 3.
        \item If $B_{n-K}=0$, set $n^{\text{active}}(n) = n^{\text{active}}(n-1) + 1$ and select arm $A_n$ according to the rule
        \begin{equation}
            A_{n} = 
            \begin{cases}
            \arg\min_a N_a^{\text{active}}(n-1), & \min_{a} N_a^{\text{active}}(n-1) < f(n^{\text{active}}(n-1)), \\
            b_{n^{\text{active}}(n)}, & \min_{a} N_a^{\text{active}}(n-1) \geq f(n^{\text{active}}(n-1)).
            \end{cases}
            \label{eq:sampling-rule}
        \end{equation}
        Set $N_a^{\text{active}}(n)=N_a^{\text{active}}(n-1)+1$ if $A_n=a$.
    \end{itemize}
    \item Set $N_a(n) = N_a(n-1) + 1$ if $A_n=a$.
    \item Set $n \leftarrow n+1$ and go to step 1.
\end{enumerate}
Notice that when $\max_a d_a(n)=R$, then arm $A_n=\argmax_a d_a(n)$ is selected with probability $1$. Else, if $\max_a d_a(n) < R$, then arm $A_n$ is selected uniformly randomly with probability $\eta>0$ and according to the rule in \eqref{eq:sampling-rule} with probability $1-\eta$. Therefore, the probability of selecting an arm at any given time is $ \ge \eta/K > 0$. As a consequence, we have the following result which demonstrates that under the proposed arms selection rule, each {\em valid} $(\underline{d}, \underline{i}, a)$ tuple is explored {\em sufficiently} many times.
\begin{lemma}
\label{lem:sufficient-exploration-of-dia-tuples}
Under the above arms selection rule, 
\begin{align}
     &\forall (\underline{d}, \underline{i}) \in \mathbb{S}_R, \quad \liminf_{n \to \infty} \frac{N(n, \underline{d}, \underline{i})}{n} > 0 \quad \text{a.s.}, \label{eq:liminf-N(n,d,i)-strictly-positive-drift} \\
    &\forall  a\in [K], ~ (\underline{d}, \underline{i}) \in \mathbb{V}_{R,a}, \quad \liminf_{n \to \infty} \frac{N(n, \underline{d}, \underline{i}, a)}{n} > 0 \quad \text{a.s.}. \label{eq:liminf-N(n,d,i,a)-strictly-positive-drift}
\end{align}
\end{lemma}
We further note the below result on the growth rate of the number of active arm selections. A proof of this follows straightforwardly from the proof of \cite[Lemma 17]{garivier2016optimal}
\begin{lemma}
\label{lem:lower-bound-on-active-arm-pulls}
The proposed arms selection rule ensures that $N_a^{\text{active}}(n) \geq (\sqrt{n^{\text{active}}(n)} - K/2)_{+} - 1$ for all $n$ large. 
\iffalse
where 
\begin{equation}
    K(n) \coloneqq \inf\{t > n: n^{\text{active}}(t) = n^{\text{active}}(n) + K\} - n, \quad n \geq K.
    \label{eq:K-of-n}
\end{equation}
\fi
\end{lemma}
%{\color{red} Will we need a lower bound on $n-K(n)$?}

\subsection{Tracking an Arbitrary Set \texorpdfstring{$C \subseteq \Sigma_R(\boldsymbol{\theta})$}{C subset of SigmaR} via Active Selection}
For all $n \geq K$ and $(\underline{d}, \underline{i}, a) \in \mathbb{S}_R \times [K]$, let 
\begin{equation}
    N^{\text{active}}(n, \underline{d}, \underline{i}, a) = \sum_{t=K}^{n} \mathbf{1}_{\{B_{t-K}=0, \, \underline{d}(t)=\underline{d}, \, \underline{i}(t)=\underline{i}, \, A_t=a\}}
    \label{eq:N-active-of-d-i-a}
\end{equation}
denote the number of occurrences of the tuple $(\underline{d}, \underline{i}, a)$ measured only at the active selection instants of arm $a$ up to time $n$. The next result provides a specification of the sequence $\{b_1, b_2, \ldots\}$ appearing in \eqref{eq:sampling-rule}.
\begin{lemma}
\label{lemma:choosing-b-n} 
Fix $\boldsymbol{\theta} \in \Theta^K$ and a compact, convex set $C \subseteq \Sigma_R(\boldsymbol{\theta})$. Let $\{\nu_1, \nu_2, \ldots\} \subset \Sigma_R(\boldsymbol{\theta})$ be such that the following holds: there exists $\varepsilon \in (0,1)$ and $n_0=n_0(\varepsilon)$ such that $d_{\infty}(\nu_n, C) \leq \varepsilon$ for all $n \geq n_0$. Let
\begin{align}
    b_{n^{\text{active}}(n)}
    &= \argmin_{a \in \mathcal{V}^{\text{active}}_{n-1}} \left\lbrace \sum_{(\underline{d}, \underline{i}) \in \mathbb{S}_R} N^{\text{active}}(n-1, \underline{d}, \underline{i}, a) - \sum_{t=K}^{n-1} \ \sum_{(\underline{d}, 
    \underline{i}) \in \mathbb{S}_R} \nu_t(\underline{d}, \underline{i}, a) \, \mathbf{1}_{\{B_{t-K}=0\}} \right\rbrace,
    \label{eq:choosing-b-n}
\end{align}
with ties, if any, resolved uniformly at random, where in \eqref{eq:choosing-b-n}, \begin{equation}
    \mathcal{V}^{\text{active}}_{n-1} \coloneqq \left\lbrace a \in [K]: \sum_{t=K}^{n-1} \sum_{(\underline{d}, \underline{i}) \in \mathbb{S}_R} \nu_t(\underline{d}, \underline{i}, a) \, \mathbf{1}_{\{B_{t-K}=0\}} > 0 \right\rbrace.
    \label{eq:set-V-active-n}
\end{equation} Then, there exists $n_1=n_1(\varepsilon)$ such that 
\begin{equation}
    d_{\infty}\left(\left\lbrace \frac{N^{\text{active}}(n, \underline{d}, \underline{i}, a)}{n^{\text{active}}(n)} \right\rbrace_{(\underline{d}, \underline{i}, a)}, C \right) \leq 5(K|\mathbb{S}_R|-1) \, \varepsilon \quad \forall \, n \geq n_1, \ \ \text{a.s.}.
    \label{eq:tracking-C}
\end{equation}
\end{lemma}
\fi

Let $\hat{a}(n) \in \arg\max_{a} \hat{\eta}_a(n) $ be the estimate of the best target arm at time $n$. Then, $\hat{a} = \hat{a}(\tau)$.  We define the following events of interest:
\begin{align}
    \mathcal{E}_1 &\coloneqq \{\tau < \infty\} = \left\lbrace \exists\,  n \geq K: Z(n) \geq \zeta(n, \delta, \alpha) \right\rbrace, \label{eq:event-1-of-interest} \\
    \mathcal{E}_2 &\coloneqq \{ \eta_{\theta_{\hat{a}(n)}} < \eta_{\theta_{a^\star(\boldsymbol{\theta})}}\}. \label{eq:event-2-of-interest}
\end{align}
We then have
\begin{align}
    & P_{\boldsymbol{\theta}}(\mathcal{E}_1 \cap \mathcal{E}_2) \nonumber\\
    &\leq P_{\boldsymbol{\theta}} \left(\exists\,  n \geq K: \inf_{\boldsymbol{\lambda} \in \textsc{Alt}(\boldsymbol{\hat{\theta}}(n))} \sum_{(\underline{d}, \underline{i}) \in \mathbb{S}_R} \ \sum_{a=1}^{K} N(n, \underline{d}, \underline{i}, a) \, D_{\text{KL}}(P_{\hat{\theta}_a(n)}^{d_a}(\cdot|i_a) \| P_{\lambda_a}^{d_a}(\cdot|i_a)) \geq \zeta(n, \delta, \alpha), \, \eta_{\theta_{\hat{a}(n)}} < \eta_{\theta_{a^\star(\boldsymbol{\theta})}}\right) \nonumber\\
    &\stackrel{(a)}{\leq} P_{\boldsymbol{\theta}} \left(\exists\,  n \geq K:  \sum_{(\underline{d}, \underline{i}) \in \mathbb{S}_R} \ \sum_{a=1}^{K} \ N(n, \underline{d}, \underline{i}, a) \, D_{\text{KL}}(P_{\hat{\theta}_a(n)}^{d_a}(\cdot|i_a) \| P_{\theta_a}^{d_a}(\cdot|i_a)) \geq \zeta(n, \delta, \alpha)\right).
    \label{eq:proof-of-delta-PAC-property-4}
\end{align}
We now note the below result on Kullback--Leibler divergences.
\begin{lemma}
\label{lem:kullback-leibler-property}
Let $S=|\mathcal{S}|$. For any $d \geq 1$, $i \in \mathcal{S}$, and $\theta, \lambda \in \Theta$, 
\begin{equation}
    D_{\text{KL}}(P_\theta^d (\cdot|i) \| P_\lambda^d (\cdot|i)) \leq d \, D_{\text{KL}}(P_\theta \| P_\lambda | \mu_\theta) + \sum_{k \in \mathcal{S}} ((I_S - P_\theta^d)(I_S - P_\theta + W_\theta)^{-1})(k|i) \, D_{\text{KL}}(P_\theta (\cdot|k) \| P_\lambda (\cdot|k)),
    \label{eq:kullback-leibler-divergence-property}
\end{equation}
where $D_{\text{KL}}(P_\theta \| P_\lambda | \mu_\theta) \coloneqq \sum_{k \in \mathcal{S}} \mu_\theta(k) \, D_{\text{KL}}(P_\theta (\cdot|k) \| P_\lambda (\cdot|k))$, $I_S$ denotes the $S \times S$ identity matrix, and $W_\theta$ denotes the matrix each of whose rows is equal to $\mu_\theta$. 
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:kullback-leibler-property}]
First, we note that
\begin{align}
    D_{\text{KL}}(P_\theta^d (\cdot|i) \| P_\lambda^d (\cdot|i)) 
    &= \sum_{j \in \mathcal{S}} P_\theta^d (j|i) \log \frac{P_\theta^d (j|i)}{P_\lambda^d (j|i)} \nonumber\\
    &=\sum_{j \in \mathcal{S}}\, \sum_{k \in \mathcal{S}} P_\theta^{d-1}(k|i) \, P_\theta(j|k) \log \frac{\sum_{k \in \mathcal{S}} P_\theta^{d-1}(k|i) \, P_\theta(j|k)}{\sum_{k \in \mathcal{S}} P_\lambda^{d-1}(k|i) \, P_\lambda(j|k)} \nonumber\\
    &\stackrel{(a)}{\leq}  \sum_{j \in \mathcal{S}}\, \sum_{k \in \mathcal{S}} P_\theta^{d-1}(k|i) \, P_\theta(j|k) \log \frac{P_\theta^{d-1}(k|i) \, P_\theta(j|k)}{P_\lambda^{d-1}(k|i) \, P_\lambda(j|k)} \nonumber\\
    &= D_{\text{KL}}(P_\theta^{d-1} (\cdot|i) \| P_\lambda^{d-1} (\cdot|i)) + \sum_{k \in \mathcal{S}} P_\theta^{d-1}(k|i) \, D_{\text{KL}}(P_\theta (\cdot|k) \| P_\lambda (\cdot|k)),
    \label{eq:proof-of-KL-divergence-property-1}
\end{align}
where $(a)$ above follows from the log-sum inequality \cite[Theorem 2.7.1]{Cover2006}. Applying the principle of induction, and using the notation $P_\theta^0=I_S$, we get
\begin{equation}
    D_{\text{KL}}(P_\theta^d (\cdot|i) \| P_\lambda^d (\cdot|i)) \leq \sum_{k \in \mathcal{S}} \left(\sum_{m=0}^{d-1} P_\theta^m(k|i)\right) \, D_{\text{KL}}(P_\theta (\cdot|k) \| P_\lambda (\cdot|k)).
    \label{eq:proof-of-KL-divergence-property-2}
\end{equation}
From \cite[Chapter 11, Exercise 16]{grinstead2006introduction}, we note the following relation:
\begin{equation}
    \left(\sum_{m=0}^{d-1} P_\theta^m \right)(I_S-P_\theta+W_\theta) = I_S - P_\theta^d + d\, W_\theta.
    \label{eq:proof-of-KL-divergence-property-3}
\end{equation}
Furthermore, from \cite[Proposition 11.1]{grinstead2006introduction}, we note that $I_S-P_\theta+W_\theta$ is invertible. Therefore, 
\begin{align}
    \sum_{m=0}^{d-1} P_\theta^m 
    &= (I_S-P_\theta^d + d\, W_\theta)(I_S-P_\theta+W_\theta)^{-1} \nonumber\\
    &=(I_S-P_\theta^d)(I_S-P_\theta+W_\theta)^{-1} + d\, W_\theta(I_S-P_\theta+W_\theta)^{-1} \nonumber\\
    &=(I_S-P_\theta^d)(I_S-P_\theta+W_\theta)^{-1} + d\, W_\theta,
    \label{eq:proof-of-KL-divergence-property-4}
\end{align}
where the last line follows by noting that
\begin{equation}
    W_\theta(I_S-P_\theta+W_\theta) = W_\theta - W_\theta\, P_\theta + W_\theta^2 = W_\theta - W_\theta + W_\theta = W_\theta.
    \label{eq:proof-of-KL-divergence-property-5}
\end{equation}
Using \eqref{eq:proof-of-KL-divergence-property-4} in \eqref{eq:proof-of-KL-divergence-property-2}, and noting that $W_\theta(k|i)=\mu_\theta(k)$ for all $(k,i)$, we arrive at \eqref{eq:kullback-leibler-divergence-property}.
\end{proof}

Using Lemma~\ref{lem:kullback-leibler-property} in \eqref{eq:proof-of-delta-PAC-property-4}, we get
\begin{align}
    & P_{\boldsymbol{\theta}}(\mathcal{E}_1 \cap \mathcal{E}_2) \nonumber\\
    &\leq P_{\boldsymbol{\theta}} \bigg(\exists\,  n \geq K:  \nonumber\\
    & {\color{black} \sum_{(\underline{d}, \underline{i}) \in \mathbb{S}_R} \ \sum_{a=1}^{K} N(n, \underline{d}, \underline{i}, a) \, \sum_{k \in \mathcal{S}} ((I_S - P_{\hat{\theta}_a(n)}^{d_a})(I_S - P_{\hat{\theta}_a(n)} + W_{\hat{\theta}_a(n)})^{-1})(k|i_a) \, D_{\text{KL}}(P_{\hat{\theta}_a(n)} (\cdot|k) \| P_{\theta_a} (\cdot|k))} \nonumber\\
    &\hspace{5cm} + \sum_{(\underline{d}, \underline{i}) \in \mathbb{S}_R} \ \sum_{a=1}^{K} \ N(n, \underline{d}, \underline{i}, a) \, d_a \, D_{\text{KL}}(P_{\hat{\theta}_a(n)} \| P_{\theta_a} \mid \mu_{\hat{\theta}_a(n)}) \geq \zeta(n, \delta, \alpha)\bigg) \nonumber\\
    &\stackrel{(a)}{\leq} P_{\boldsymbol{\theta}} \bigg(\exists\,  n \geq K:  \nonumber\\
    & {\color{black} \sum_{(\underline{d}, \underline{i}) \in \mathbb{S}_R} \ \sum_{a=1}^{K} N(n, \underline{d}, \underline{i}, a) \, \sum_{k \in \mathcal{S}} ((I_S - P_{\hat{\theta}_a(n)}^{d_a}) (I_S - P_{\hat{\theta}_a(n)} + W_{\hat{\theta}_a(n)})^{-1})(k|i_a) \, D_{\text{KL}}(P_{\hat{\theta}_a(n)} (\cdot|k) \| P_{\theta_a} (\cdot|k))} \nonumber\\
    &\hspace{8cm} + \sum_{a=1}^{K} n \, D_{\text{KL}}(P_{\hat{\theta}_a(n)} \| P_{\theta_a} \mid \mu_{\hat{\theta}_a(n)}) \geq \zeta(n, \delta, \alpha)\bigg),
    \label{eq:proof-of-delta-PAC-property-5}
\end{align}
where in writing $(a)$ above, we use the important property
\begin{equation}
    \sum_{(\underline{d}, \underline{i}) \in \mathbb{S}_R} d_a\, N(n, \underline{d}, \underline{i}, a) \leq n \quad \forall \, a \in [K];
    \label{eq:an-important-property-of-restless-chains}
\end{equation}
see, for instance, \cite[Appendix G]{karthik2021detecting} and the discussion therein. 

We now note that for all $i, k \in \mathcal{S}$,
\begin{align}
    ((I_S - P_{\hat{\theta}_a(n)}^{d})(I_S - P_{\hat{\theta}_a(n)}+ W_{\hat{\theta}_a(n)})^{-1})(k|i) 
    &= \sum_{m=0}^{d-1} P_{\hat{\theta}_a(n)}^m (k|i) - d \, W_{\hat{\theta}_a(n)}(k|i)
    \leq d.
\end{align}
We then have (again using \eqref{eq:an-important-property-of-restless-chains})
\begin{align}
    & P_{\boldsymbol{\theta}}(\mathcal{E}_1 \cap \mathcal{E}_2)  \nonumber\\
    &\leq P_{\boldsymbol{\theta}} \bigg(\exists\,  n \geq K:  {\color{black} \sum_{(\underline{d}, \underline{i}) \in \mathbb{S}_R} \ \sum_{a=1}^{K} d_a \, N(n, \underline{d}, \underline{i}, a) \sum_{k \in \mathcal{S}} D_{\text{KL}}(P_{\hat{\theta}_a(n)} (\cdot|k) \| P_{\theta_a} (\cdot|k))} \nonumber\\
    &\hspace{8cm} + \sum_{a=1}^{K} n \, D_{\text{KL}}(P_{\hat{\theta}_a(n)} \| P_{\theta_a} \mid \mu_{\hat{\theta}_a(n)}) \geq \zeta(n, \delta, \alpha)\bigg) \nonumber\\
    &\leq P_{\boldsymbol{\theta}} \bigg(\exists\,  n \geq K: \sum_{a=1}^{K} {\color{black} n \sum_{k \in \mathcal{S}} D_{\text{KL}}(P_{\hat{\theta}_a(n)} (\cdot|k) \| P_{\theta_a} (\cdot|k))} + \sum_{a=1}^{K} \, n
    \, D_{\text{KL}}(P_{\hat{\theta}_a(n)} \| P_{\theta_a} \mid \mu_{\hat{\theta}_a(n)}) \geq \zeta(n, \delta, \alpha) \bigg) \nonumber\\
    &=P_{\boldsymbol{\theta}} \bigg(\exists\,  n \geq K: \sum_{a=1}^{K} {\color{black} n \sum_{k \in \mathcal{S}} \frac{1}{\mu_{\hat{\theta}_a(n)}(k)} \, \mu_{\hat{\theta}_a(n)}(k) \, D_{\text{KL}}(P_{\hat{\theta}_a(n)} (\cdot|k) \| P_{\theta_a} (\cdot|k))} \nonumber\\
    &\hspace{8cm} + \sum_{a=1}^{K} \, n
    \, D_{\text{KL}}(P_{\hat{\theta}_a(n)} \| P_{\theta_a} \mid \mu_{\hat{\theta}_a(n)}) \geq \zeta(n, \delta, \alpha) \bigg) \nonumber\\
    &\stackrel{(a)}{\leq} P_{\boldsymbol{\theta}} \bigg(\exists\,  n \geq K: \sum_{a=1}^{K} {\color{black} \frac{n}{\gamma} \, D_{\text{KL}}(P_{\hat{\theta}_a(n)} \| P_{\theta_a} \mid \mu_{\hat{\theta}_a(n)})} + \sum_{a=1}^{K} \, n
    \, D_{\text{KL}}(P_{\hat{\theta}_a(n)} \| P_{\theta_a} \mid \mu_{\hat{\theta}_a(n)}) \geq \zeta(n, \delta, \alpha) \bigg) \nonumber\\
    &\leq \sum_{n=K}^{\infty} P_{\boldsymbol{\theta}} \bigg(\sum_{a=1}^{K} {\color{black} n \, D_{\text{KL}}(P_{\hat{\theta}_a(n)} \| P_{\theta_a} \mid \mu_{\hat{\theta}_a(n)})} \geq \frac{\zeta(n, \delta, \alpha)}{1+\frac{1}{\gamma}} \bigg) \nonumber\\
    &\leq \sum_{n=K}^{\infty} \ \sum_{a=1}^{K} P_{\boldsymbol{\theta}} \bigg({\color{black} n \, D_{\text{KL}}(P_{\hat{\theta}_a(n)} \| P_{\theta_a} \mid \mu_{\hat{\theta}_a(n)})} \geq \frac{\zeta(n, \delta, \alpha)}{K \big(1+\frac{1}{\gamma}\big)} \bigg) \nonumber\\
    &=\sum_{n=K}^{\infty} \ \sum_{a=1}^{K} P_{\boldsymbol{\theta}} \bigg({\color{black} n \, D_{\text{KL}}(P_{\hat{\theta}_a(n)} \| P_{\theta_a} \mid \mu_{\hat{\theta}_a(n)})} \geq \log\left(\frac{D\, n^\alpha}{\delta}\right) \bigg) \nonumber\\
    &\leq \delta.
\end{align}
In the above set of inequalities, $(a)$ follows by noting that $\mu_{\hat{\theta}_a(n)}(k) \geq \gamma$ for all $k \in \mathcal{S}$ and $n \geq K$ (by the definition of $\gamma$), and the last line results from following the lines of the proof of \cite[Lemma 14, Appendix 4.B]{moulos2019optimal}.





\iffalse
Fix $a \in [K]$, and consider the ``error'' term
\begin{align}
    &\sum_{(\underline{d}, \underline{i}) \in \mathbb{S}_R} \, N(n, \underline{d}, \underline{i}, a) \, \sum_{k \in \mathcal{S}} \, ((I_S - P_{\hat{\theta}_a(n)}^{d_a})(I_S - P_{\hat{\theta}_a(n)} + W_{\hat{\theta}_a(n)})^{-1})(k|i_a) \, D_{\text{KL}}(P_{\hat{\theta}_a(n)} (\cdot|k) \| P_{\theta_a} (\cdot|k)) \nonumber\\
    &= \sum_{k \in \mathcal{S}} \, \sum_{d=1}^{R} \, \sum_{i \in \mathcal{S}} \, N(n, d, i, a) \, ((I_S - P_{\hat{\theta}_a(n)}^{d})(I_S - P_{\hat{\theta}_a(n)} + W_{\hat{\theta}_a(n)})^{-1})(k|i) \, D_{\text{KL}}(P_{\hat{\theta}_a(n)} (\cdot|k) \| P_{\theta_a} (\cdot|k)) \nonumber\\
    &= \sum_{d=1}^{R} \mathbf{a}_{n,d}^\top \, (I_S - P_{\hat{\theta}_a(n)}^{d})(I_S - P_{\hat{\theta}_a(n)} + W_{\hat{\theta}_a(n)})^{-1}\, \mathbf{v},
\end{align}
where $N(n, d, i, a) = \sum_{t=K}^{n} \mathbf{1}_{\{ d_a(t)=d, \, i_a(t)=i, \, A_t=a \}} = \sum_{t=K}^{n} \mathbf{1}_{\{X_{t-d_a}^a = i, \, A_t=a\}}$, 
$$
\mathbf{a}_{n,d} = [N(n, d, i, a)]_{i \in \mathcal{S}}, \quad \mathbf{v} = [D_{\text{KL}}(P_{\hat{\theta}_a(n)} (\cdot|k) \| P_{\theta_a} (\cdot|k))]_{k \in \mathcal{S}}.
$$
\fi

\iffalse
As a consequence of Lemma~\ref{lem:kullback-leibler-property}, we have
\begin{align}
    P_{\boldsymbol{\theta}}(\mathcal{E}_1 \cap \mathcal{E}_2) &\leq P_{\boldsymbol{\theta}} \left(\exists\,  n \geq K:  \sum_{(\underline{d}, \underline{i}) \in \mathbb{S}_R} \ \sum_{a=1}^{K} \ \frac{d_a}{\mu_{\hat{\theta}_a(n)}(i_a)} \, N(n, \underline{d}, \underline{i}, a) \, D_{\text{KL}}(P_{\hat{\theta}_a(n)} \| P_{\theta_a} | \mu_{\hat{\theta}_a(n)}) \geq \zeta(n, \delta, \alpha)\right) \nonumber\\
    &\stackrel{(b)}{\leq} P_{\boldsymbol{\theta}} \left(\exists\,  n \geq K:  \sum_{a=1}^{K} n\, D_{\text{KL}}(P_{\hat{\theta}_a(n)} \| P_{\theta_a} | \mu_{\hat{\theta}_a(n)}) \geq \zeta(n, \delta, \alpha) \, C_{\hat{\boldsymbol{\theta}}(n)}\right) \nonumber\\
    &\stackrel{(c)}{\leq} \sum_{a=1}^{K} P_{\boldsymbol{\theta}} \left(\exists\,  n \geq K:\ n\, D_{\text{KL}}(P_{\hat{\theta}_a(n)} \| P_{\theta_a} | \mu_{\hat{\theta}_a(n)}) \geq \frac{C_{\hat{\boldsymbol{\theta}}(n)}}{K}\, \zeta(n, \delta, \alpha)\right) \nonumber\\
    &=\sum_{a=1}^{K} P_{\boldsymbol{\theta}} \left(\exists\,  n \geq K:\ n\, D_{\text{KL}}(P_{\hat{\theta}_a(n)} \| P_{\theta_a} | \mu_{\hat{\theta}_a(n)}) \geq \frac{2\,n_0}{n_0-1}\, \log\log n + n_0\right),
\end{align}
where in writing $(b)$ above, we use the important observation that
$$
\sum_{(\underline{d}, \underline{i}) \in \mathbb{S}_R} \ d_a \, N(n, \underline{d}, \underline{i}, a) \leq n.
$$ for all $a \in [K]$, and $(c)$ above follows from the union bound. Using the law of iterated logarithms for Markov chains \cite[Chapter~3, Theorem~11]{moulosanantharam2019optimal}, we get
\begin{align}
    P_{\boldsymbol{\theta}}(\mathcal{E}_1 \cap \mathcal{E}_2)
    &\leq \sum_{a=1}^{K} 4K^\prime e\,n_0^2\,\exp(-n_0)\nonumber\\
    &=4KK^\prime e\,n_0^2\,\exp(-n_0)\nonumber\\
    &\leq \delta,
    \label{eq:proof-of-delta-PAC-property-5}
\end{align}
where the last line follows from the definition of $n_0$ (see \eqref{eq:n-0-definition}). This completes the proof.
\fi 


%---------------------------------------------------------------------------------------------------------------------------------------------

\iffalse
\section{Proof of Proposition~\ref{prop:almost-sure-upper-bound}}

We use the below technical lemma from \cite{garivier2016optimal} in the proof.
\begin{lemma}
\label{lemma:technical-lemma}\cite[Lemma 18]{garivier2016optimal}
For any two constants $c_1>0, c_2>0$ such that $c_2/c_1 \geq 1$ and $\rho \geq 0$, 
\begin{equation}
    \inf\{n \geq 1: n c_1 \geq \log(c_2 n^{1+\rho})\} \leq \frac{1+\rho}{c_1} \left(\log\frac{c_2 e}{c_1^{1+\rho}} + \log\log \frac{c_2}{c_1^{1+\rho}}\right).
\end{equation}
\end{lemma}
Fix a problem instance $\boldsymbol{\theta}$ such that $a^\star(\boldsymbol{\theta})$ is unique, and consider the event
\begin{equation}
    \mathcal{E} = \left\lbrace d_{\infty}((N(n, \underline{d}, \underline{i}, a)/n)_{(\underline{d}, \underline{i}, a)}, \ C_\gamma^\star(\boldsymbol{\theta})) \stackrel{n \to \infty}{\longrightarrow} 0, \quad  \hat{\boldsymbol{\eta}}(n) \stackrel{n \to \infty}{\longrightarrow} \boldsymbol{\eta}, \quad  \hat{\boldsymbol{\theta}}(n) \stackrel{n \to \infty}{\longrightarrow} \boldsymbol{\theta} \right\rbrace.
    \label{eq:event-of-interest-almost-sure-upper-bound}
\end{equation}
From Lemma \ref{lem:convergence-of-ML-estimates} and Lemma~\ref{lem:convergence-to-the-correct-set-of-optimal-allocations}, we know that $\mathcal{E}$ occurs with probability $1$ under our policy.
Fix $\varepsilon>0$ and $\nu^\star \in C_\gamma^\star(\boldsymbol{\theta})$ arbitrarily. From the continuity of $\psi$ (Lemma~\ref{lem:attainment-of-supremum}), we know that there exists an open neighbourhood of $\{\boldsymbol{\theta}\} \times C_\gamma^\star(\boldsymbol{\theta})$, say $\mathcal{U}=\mathcal{U}(\varepsilon)$, such that
\begin{equation}
    \psi(\boldsymbol{\lambda}, \nu^\prime) \geq (1-\varepsilon)\, \psi(\boldsymbol{\theta}, \nu^\star) = (1-\varepsilon)\, (\gamma\, T_R^{\text{unif}}(\boldsymbol{\theta})+ (1-\gamma)\, T_R^\star(\boldsymbol{\theta})) \quad \forall (\boldsymbol{\lambda}, \nu^\prime) \in \mathcal{U}.
\end{equation}
Under the event $\mathcal{E}$, there exists $N_0 = N_0(\varepsilon)$ such that $(\hat{\boldsymbol{\mu}}(n), (N_i(n)/n)_{i \in [S]}) \in \mathcal{U}$ for all $n \geq N_0$, and consequently
\begin{equation}
    \psi(\hat{\boldsymbol{\mu}}(n), (N_i(n)/n)_{i \in [S]}) \geq (1-\varepsilon)\, (1-\varepsilon)\, (\gamma\, T_R^{\text{unif}}(\boldsymbol{\theta})+ (1-\gamma)\, T_R^\star(\boldsymbol{\theta})) \quad \forall n \geq N_0.
\end{equation}
Note that
$$
    Z(n) = n \, \psi(\hat{\boldsymbol{\theta}}(n), (N(n, \underline{d}, \underline{i},  a)/n)_{(\underline{d}, \underline{i}, a))}) \geq n(1-\varepsilon)(1-\varepsilon)\, (\gamma\, T_R^{\text{unif}}(\boldsymbol{\theta})+ (1-\gamma)\, T_R^\star(\boldsymbol{\theta})) \quad \forall n \geq N_0.
$$
We then have
\begin{align}
    \tau_{\delta}
    &= \inf\left\lbrace n \geq K: Z(n) \geq \zeta(n, \delta, \alpha)    \right\rbrace \nonumber\\
    & \leq \inf\left\lbrace n \geq \max\{N_0, K\}: n\,(1-\varepsilon)\, (\gamma\, T_R^{\text{unif}}(\boldsymbol{\theta})+ (1-\gamma)\, T_R^\star(\boldsymbol{\theta})) \geq \frac{K}{C_{\hat{\boldsymbol{\theta}}(n)}} \left[\frac{2\,n_0}{n_0-1}\, \log\log n + n_0\right] \right\rbrace.
    \label{eq:proof-of-almost-sure-upper-bound-2}
\end{align}
Under the instance $\boldsymbol{\theta} \in \Theta^K$, we note that $C_{\hat{\boldsymbol{\theta}}(n)} \to C_{\boldsymbol{\theta}} = \min_a \min_i \mu_{\theta_a}(i)>0$ a.s. as $n \to \infty$. Fix $\varepsilon^\prime>0$ satisfying $\log(1+\varepsilon^\prime) < \frac{C_{\boldsymbol{\theta}}}{2K}$. Then, there exists $N_1 \geq K$ a.s. finite such that
\begin{equation}
    C_{\hat{\boldsymbol{\theta}}(n)} \geq \frac{C_{\boldsymbol{\theta}}}{2 \, \log\left(1+\varepsilon^\prime\right)} \quad \forall n \geq N_1.
\end{equation}
We then have
\begin{align}
    \tau_{\delta}
    &\leq \inf \bigg\lbrace n \geq \max\{N_0, N_1, K\}: n(1-\varepsilon)\, (\gamma\, T_R^{\text{unif}}(\boldsymbol{\theta})+ (1-\gamma)\, T_R^\star(\boldsymbol{\theta})) \nonumber\\
    &\hspace{7cm}\geq \frac{2K\, \log\left(1+\varepsilon^\prime\right)}{C_{\boldsymbol{\theta}}} \left[\frac{2\,n_0}{n_0-1}\, \log\log n + n_0\right] \bigg\rbrace.
    \label{eq:proof-of-almost-sure-upper-bound-3}
\end{align}
Let $N_2 \coloneqq \inf\left\lbrace n > 1: \log\left(\frac{n}{\delta}\right) \geq \frac{2K\, \log\left(1+\varepsilon^\prime\right)}{C_{\boldsymbol{\theta}}} \left[\frac{2\,n_0}{n_0-1}\, \log\log n + n_0\right]\right\rbrace$. Then, we have
\begin{align}
    \tau_{\delta}
    &\leq \inf \left\lbrace n \geq \max\{N_0, N_1, N_2, K\}: n\,(1-\varepsilon)\, (\gamma\, T_R^{\text{unif}}(\boldsymbol{\theta})+ (1-\gamma)\, T_R^\star(\boldsymbol{\theta})) \geq \log\left(\frac{n}{\delta}\right) \right\rbrace \nonumber\\
    &\leq \max\left\lbrace N_0, N_1, N_2, K, \quad \frac{1}{(1-\varepsilon)\, (\gamma\, T_R^{\text{unif}}(\boldsymbol{\theta})+ (1-\gamma)\, T_R^\star(\boldsymbol{\theta}))} \log\frac{1}{\delta} + o(\log(1/\delta))\right\rbrace
    \label{eq:proof-of-almost-sure-upper-bound-4}
\end{align}
for all $\delta$ sufficiently small, where the last line above follows from the application of Lemma \ref{lemma:technical-lemma} with
$$
c_1 = (1-\varepsilon)(\gamma\, T_R^{\text{unif}}(\boldsymbol{\theta})+ (1-\gamma)\, T_R^\star(\boldsymbol{\theta})), \quad c_2 = \frac{1}{\delta}, \quad \rho=0.
$$
Eq. \eqref{eq:proof-of-almost-sure-upper-bound-4} immediately yields $P_{\boldsymbol{\theta}}(\tau_{\delta} < \infty)=1$. Noting that the maximum of non-negative terms may be upper bounded by their sum, we get
\begin{align}
    \frac{\tau_{\delta}}{\log(1/\delta)} \leq \frac{K+ N_0 + N_1}{\log(1/\delta)} + \frac{N_2}{\log(1/\delta)} + \frac{1}{(1-\varepsilon)\, (\gamma\, T_R^{\text{unif}}(\boldsymbol{\theta})+ (1-\gamma)\, T_R^\star(\boldsymbol{\theta}))} + \frac{o(\log(1/\delta))}{\log(1/\delta)}.
    \label{eq:proof-of-almost-sure-upper-bound-5}
\end{align}
Noting that $K$, $N_0$, and $N_1$ do not depend on $\delta$, and using the fact that the last term on the right-hand side of \eqref{eq:proof-of-almost-sure-upper-bound-5} converges to $0$ in the limit as $\delta \downarrow 0$, we get
\begin{equation}
    \limsup_{\delta \downarrow 0} \frac{\tau_\delta}{\log(1/\delta)} \leq \limsup_{\delta \downarrow 0} \frac{N_2}{\log(1/\delta)} + \frac{1}{(1-\varepsilon)\, (\gamma\, T_R^{\text{unif}}(\boldsymbol{\theta})+ (1-\gamma)\, T_R^\star(\boldsymbol{\theta}))}.
    \label{eq:proof-of-almost-sure-upper-bound-6}
\end{equation}
We now claim that the first term on the right-hand side of \eqref{eq:proof-of-almost-sure-upper-bound-6} is equal to $0$. Assuming that the claim is true, taking limits as $\varepsilon\downarrow 0$, we arrive at \eqref{eq:almost-sure-upper-bound}. To show the claim, we first note from \eqref{eq:n-0-definition} that $n_0 \to \infty$ as $\delta \downarrow 0$, and hence $\frac{n_0}{n_0-1} \to 1$ as $\delta \downarrow 0$. This implies that there exists $C_1$ such that $\frac{n_0}{n_0-1} \leq C_1$ for all $\delta > 0$. Furthermore, we note from \eqref{eq:n-0-definition} that
\begin{align}
    n_0 
    &= \inf\bigg\lbrace n \geq K: n^2 e^{-n} \leq \frac{\delta}{4KK^\prime \, e} \bigg\rbrace \nonumber\\
    &\stackrel{(a)}{\leq} \inf\bigg\lbrace n \geq N_3: \left(1+\varepsilon^\prime\right)^{-n\, \frac{2K}{C_{\boldsymbol{\theta}}}} \leq \frac{\delta}{4KK^\prime \, e} \bigg\rbrace \nonumber\\
    &\leq N_3 + \bigg\lceil \frac{C_{\boldsymbol{\theta}}}{2K}\, \frac{\log\left(\frac{4KK^\prime\, e}{\delta}\right)}{\log\left(1+\varepsilon^\prime\right)} \bigg\rceil \nonumber\\
    &\leq N_3 + \frac{C_{\boldsymbol{\theta}}}{2K}\, \frac{\log\left(\frac{4KK^\prime\, e}{\delta}\right)}{\log\left(1+\varepsilon^\prime\right)} + 1,
    \label{eq:proof-of-almost-sure-upper-bound-7}
\end{align}
where in $(a)$ above, $N_3 \coloneqq \inf\{n \geq K: n^2 e^{-n} \leq \left(1+\varepsilon^\prime\right)^{-n\, \frac{2K}{C_{\boldsymbol{\theta}}}}\}$. Note that $N_3 < +\infty$ by definition of $\varepsilon^\prime$. We then have
\begin{align}
    N_2
    &= \inf\left\lbrace n > 1: \log\left(\frac{n}{\delta}\right) \geq \frac{2K\, \log\left(1+\varepsilon^\prime\right)}{C_{\boldsymbol{\theta}}} \left[\frac{2\,n_0}{n_0-1}\, \log\log n + n_0\right]\right\rbrace \nonumber\\
    &\leq \inf\left\lbrace n > 1: \log\left(\frac{n}{\delta}\right) \geq \frac{2K\, \log\left(1+\varepsilon^\prime\right)}{C_{\boldsymbol{\theta}}} \left[2C_1\, \log\log n + n_0\right]\right\rbrace \nonumber\\
    &\leq \inf\left\lbrace n > 1: \log\left(\frac{n}{\delta}\right) \geq \frac{4K\,C_1\, \log\left(1+\varepsilon^\prime\right)}{C_{\boldsymbol{\theta}}}\, \log\log n + \log\left(\frac{4KK^\prime\, e}{\delta}\right) + (N_3+1)\,\frac{2K\, \log\left(1+\varepsilon^\prime\right)}{C_{\boldsymbol{\theta}}}\right\rbrace \nonumber\\
    &= \inf\left\lbrace n > 1: \log n \geq \frac{4K\,C_1\, \log\left(1+\varepsilon^\prime\right)}{C_{\boldsymbol{\theta}}}\, \log\log n + \log (4KK^\prime\,e) + (N_3+1)\,\frac{2K\, \log\left(1+\varepsilon^\prime\right)}{C_{\boldsymbol{\theta}}}\right\rbrace.
    \label{eq:proof-of-almost-sure-upper-bound-8}
\end{align}
Dividing both sides of \eqref{eq:proof-of-almost-sure-upper-bound-8} by $\log(1/\delta)$ and noting that the right-hand side of \eqref{eq:proof-of-almost-sure-upper-bound-8} does not depend on $\delta$, we get $\limsup_{\delta \downarrow 0} \frac{N_2}{\log(1/\delta)} = 0$. This completes the proof.
\fi

==> setting.tex <==
\section{setting}


==> srs-policies-and-ergodicity.tex <==
\section{Stationary Randomised Strategies and a Key Ergodicity Property}

Under an arbitrary policy $\pi$, the action $A_t$ may, in general, be chosen based on the history $\mathcal{F}_t$ for each $t\geq K$. In the special case when $A_t$ is chosen based only on the current state $(\underline{d}(t), \underline{i}(t))$ for all $t\geq K$, the controlled Markov process $\{(\underline{d}(t), \underline{i}(t)):\ t\geq K\}$ is, in fact, a Markov process. To see this, note that
\begin{align}
&P_C^\pi(\underline{d}(t+1)=\underline{d}',\underline{i}(t+1)=\underline{i}'\mid \{(\underline{d}(s),\underline{i}(s)), \ K\leq s \leq t\})\nonumber\\
&=\sum_{a=1}^{K}\ P_C^\pi(\underline{d}(t+1)=\underline{d}',\underline{i}(t+1)=\underline{i}', A_t=a\mid \{(\underline{d}(s),\underline{i}(s)), \ K\leq s \leq t\})\nonumber\\
&\stackrel{(a)}{=}\sum_{a=1}^{K}\ P_C^\pi(A_t=a\mid \{(\underline{d}(s),\underline{i}(s)), \ K\leq s \leq t\}) \cdot Q_{C}(\underline{d}', \underline{i}'|\underline{d}(t), \underline{i}(t), a)\nonumber\\
&=\sum_{a=1}^{K}\ P_C^\pi(A_t=a\mid \underline{d}(t),\underline{i}(t)) \cdot Q_{C}(\underline{d}', \underline{i}'|\underline{d}(t), \underline{i}(t), a)\nonumber\\
&=P_C^\pi(\underline{d}(t+1)=\underline{d}',\underline{i}(t+1)=\underline{i}'\mid \underline{d}(t),\underline{i}(t)),
\label{eq:A_t_is_selected_based_on_d(t)_i(t)_only}
\end{align}
where $(a)$ above follows from \eqref{eq:controlled_markov_chain}.

Call $\pi$ a {\em stationary randomised strategy} (or SRS policy) if there exists $\lambda=\bigotimes _{(\underline{d},\underline{i})\in\mathbb{S}} \lambda(\cdot \mid\underline{d},\underline{i})$, with the component $\lambda(\cdot \mid\underline{d},\underline{i})$ being a probability distribution on $\mathcal{A}$ for each $(\underline{d},\underline{i})\in \mathbb{S}$, such that 
\begin{equation}
P_C^\pi(A_t=a\mid \mathcal{F}_t)=\lambda(a|\underline{d}(t),\underline{i}(t)) \quad \forall \ t\geq K.
\label{eq:SRS_policy}
\end{equation}
Let the SRS policy in \eqref{eq:SRS_policy} be denoted explicitly as $\pi^\lambda$, and let $\Pi_{\textsf{SRS}}$ denote the space of all SRS policies. If the process $\{(\underline{d}(t), \underline{i}(t)):\ t\geq K\}$ is ergodic under the SRS policy $\pi^{\lambda}$, it possesses a unique stationary distribution which we denote by $\mu^\lambda=\{\mu^\lambda(\underline{d}, \underline{i}):\ (\underline{d}, \underline{i})\in \mathbb{S}\}$. Further, we write 
\begin{equation}
\nu^\lambda(\underline{d}, \underline{i}, a) \coloneqq \mu^\lambda(\underline{d}, \underline{i}) \ \lambda(a|\underline{d}, \underline{i}), \quad (\underline{d}, \underline{i})\in \mathbb{S}, \ a\in \mathcal{A},
\label{eq:ergodic_state_action_occupancy_measure}
\end{equation}
to denote the {\em ergodic state-action occupancy} measure under $\pi^\lambda$. We write $\pi^{\textsf{unif}}$ to denote the SRS policy defined by
\begin{equation}
\lambda_{\textsf{unif}}(a|\underline{d}, \underline{i})=\frac{1}{K}, \quad a\in \mathcal{A}, \ (\underline{d}, \underline{i})\in \mathbb{S}.
\label{eq:unif-SRS-policy}
\end{equation}

The below result demonstrates that the process $\{(\underline{d}(t), \underline{i}(t)):\ t\geq K\}$ is ergodic under $\pi^{\textsf{unif}}$.
\begin{lemma}
\label{lemma:ergodicity-under-unif-SRS-policy}
For each $C\in \mathcal{C}$, the process $\{(\underline{d}(t), \underline{i}(t)):\ t\geq K\}$ is ergodic under the SRS policy $\pi^{\textsf{unif}}$ and under the TPMs assignment $C$.
\end{lemma}
\begin{IEEEproof}
See Appendix \ref{appndx:proof-of-lemma-ergodicity-under-unif-SRS-policy}.
\end{IEEEproof}
As a consequence of Lemma \ref{lemma:ergodicity-under-unif-SRS-policy}, the process $\{(\underline{d}(t), \underline{i}(t)):\ t\geq K\}$ has a unique stationary distribution, say $\mu_{C}^{\textsf{unif}}=\{\mu_{C}^{\textsf{unif}}(\underline{d}, \underline{i}): (\underline{d}, \underline{i})\in \mathbb{S}\}$, under the SRS policy $\pi^{\textsf{unif}}$ and under the TPMs assignment $C$. We note that $\mu_{C}^{\textsf{unif}}(\underline{d}, \underline{i})>0$ for all $(\underline{d}, \underline{i})\in \mathbb{S}$. Let
\begin{align}
\nu_{C}^{\textsf{unif}}(\underline{d}, \underline{i}, a) &\coloneqq \mu_{C}^{\textsf{unif}}(\underline{d}, \underline{i})\cdot \lambda_{\textsf{unif}}(a|\underline{d}, \underline{i})\nonumber\\
&= \frac{\mu_{C}^{\textsf{unif}}(\underline{d}, \underline{i})}{K}, \quad (\underline{d}, \underline{i})\in \mathbb{S}, \ a\in \mathcal{A},
\label{eq:ergodic-state-action-under-unif}
\end{align}
denote the corresponding ergodic state-action occupancy measure. 



